Deep unfolding of MCMC kernels: scalable, modular & explainable GANs for high-dimensional posterior sampling

Markov chain Monte Carlo (MCMC) methods are fundamental to Bayesian computation, but can be computationally intensive, especially in high-dimensional settings. Push-forward generative models, such as generative adversarial networks (GANs), variational auto-encoders and normalising flows offer a computationally efficient alternative for posterior sampling. However, push-forward models are opaque as they lack the modularity of Bayes Theorem, leading to poor generalisation with respect to changes in the likelihood function. In this work, we introduce a novel approach to GAN architecture design by applying deep unfolding to Langevin MCMC algorithms. This paradigm maps fixed-step iterative algorithms onto modular neural networks, yielding architectures that are both flexible and amenable to interpretation. Crucially, our design allows key model parameters to be specified at inference time, offering robustness to changes in the likelihood parameters. We train these unfolded samplers end-to-end using a supervised regularized Wasserstein GAN framework for posterior sampling. Through extensive Bayesian imaging experiments, we demonstrate that our proposed approach achieves high sampling accuracy and excellent computational efficiency, while retaining the physics consistency, adaptability and interpretability of classical MCMC strategies.

==> figures/MNIST_results.tex <==
\begin{table}
	\centering
	\resizebox{\linewidth}{!}{
		\begin{tabular}{|c | c c c | c c c| c c|}
			\hline
			Method (NFEs) & \makecell{PSNR \\(sample)} & \makecell{PSNR \\ (mean)}  & LPIPS & \makecell{SW \\ ($\times 10^5$)}  & \makecell{$\mathcal W_2^\text{Latent}$ \\ ($\times 10^2$)} & \makecell{CMMD \\ ($\times 10^3$)} & \makecell{Time\\ (ms)} &\makecell{Size\\ (MB)} \\
			\hline
			\rowcolor{gray!12} U-SGS (4) & 23.77 & 24.96  & 0.007 & 9.53  & 3.70 & 12.70 &0.13 & \textbf{4.0} \\
			\rowcolor{gray!12}  U-SGS (8) & 24.95 & 26.29  & 0.006 & 8.49  & 2.58 & 3.91 & 0.24 & 4.0 \\
			\rowcolor{gray!12}  U-SGS (16) & 25.78 & 27.34  & 0.005 & 7.08  & 0.96 & 5.86 & 0.48 & 4.0 \\
			\rowcolor{gray!12}  U-SGS (32) & 26.93 & 28.12  & 0.003 & \textbf{6.72}  & 0.54 & 1.95 & 0.96 & 4.0 \\
			\rowcolor{gray!12}  U-SGS (64) & \textbf{27.59} & \textbf{28.46}  & \textbf{0.003} & 6.95  & \textbf{0.35} & \textbf{0.98} & 1.89 & 4.0 \\
			\hline
			RCGAN (1) & 23.28 & 26.69  & 0.009 & 9.21  & 9.08 & 21.48 & \textbf{0.10} & 11.83 \\
			\hline
			VAE-SGS ($10^4$) & 23.38 & 23.49  & 0.015 & 11.66  & 0.92 & 18.56 & 120 & 2.7 \\
			\hline
		\end{tabular}
	}
	\caption{Reconstruction metrics for the Random Motion deblurring problem. Results are averaged over the MNIST test dataset, using our unrolled Langevin model with $L=2^{i}$ iterations, $2\le i\le 6$. Comparisons are made with the rcGAN architecture \cite{bendel2023regularized} and a zero-shot split Gibbs sampler with a data-driven VAE prior (VAE-SGS). LPIPS is computed using a single approximate posterior sample from each model. For each observation $y$, PSNR results are computed for a single posterior sample and for the posterior mean, approximated using 512 Monte Carlo samples, with the exception of VAE-SGS for which the posterior mean is approximated by the ergodic average. The final columns show the time to generate a single posterior sample for each model, and the storage cost of model parameters. Metrics are scaled by the stated factors to assist readability.}
	\label{tab:mnist_metrics}
\end{table}



\begin{figure}
	\centering
	\begin{tikzpicture}
		\begin{axis}[
			name=ax1,
			xlabel=$L$,
			ylabel= Mean-Square Error,
			ymode=log,
			xmode = log,
			log basis x=2,
			log basis y=10,
			ymin=0.001,
			grid=both,
			legend style={at={(0.52,1)},anchor=south west, legend columns=-1},
			width=0.4\linewidth,
			xticklabels={,4,8,16,32,64}
			]
			\addplot[black,mark=*] table[x expr = \thisrow{L}, y expr = 10^(-\thisrow{Unrolled}/10), col sep = comma]{data/MNIST_mse.csv};
			\addlegendentry{U-SGS}
			\addplot[black,mark=square] table[x expr = \thisrow{L}, y expr = 10^(-\thisrow{VAE}/10), col sep = comma]{data/MNIST_mse.csv};
			\addlegendentry{VAE-SGS (Zero-shot)}
		\end{axis}
		\begin{axis}[
			at={(ax1.south east)},
			xshift=2cm,
			xlabel=$L$,
			ylabel= $\mathcal W_2^\text{Latent}$,
			ymode=log,
			xmode = log,
			log basis x=2,
			log basis y=10,
			grid=both,
			width=0.4\linewidth,
			xticklabels={,4,8,16,32,64}
			]
			\addplot[black,mark=*] table[x expr = \thisrow{L}, y expr = \thisrow{Unrolled_FID}, col sep = comma]{data/MNIST_mse.csv};
			\addplot[black,mark=square] table[x expr = \thisrow{L}, y expr = \thisrow{VAE_FID}, col sep = comma]{data/MNIST_mse.csv};
		\end{axis}
	\end{tikzpicture}
	\caption{Convergence comparison of U-SGS and conventional SGS on small truncated chains.}
	\label{fig:numerics/Conv_MNIST}
	%TODO: Plot gammas as well
\end{figure}

==> figures/RI_results.tex <==
\begin{table} 
	\centering

		% Validation samples
		\begin{tabular}{|c |  c c c c c| c c c|}
			\hline
			Model (NFEs) & \makecell{PSNR \\ (Sample)} & \makecell{PSNR \\ (Mean)} & LPIPS & SSIM & CFID & \makecell{Time\\ (s)} & \makecell{RAM \\ (MB)} & \makecell{Weights\\ (M)}\\
			\hline
			RIGAN (1) & 41.51 & 43.77 & 0.07 & \bf 0.91 & 0.52 & \bf 0.04 & 1078 & 195.8\\
			\rowcolor{gray!12} U-LATINO (8) & 43.40 & 45.61 & \bf 0.01  & 0.88 & \bf 0.06 & 0.08 & \bf 683 & 88.3\\
			\hline 
			LATINO (8) & 37.33 & 37.90 & 0.08 & 0.64 & 0.19 & 0.48 & \bf 683 & 88.0\\
			IRIS (1000) & \bf 48.08 & \bf 48.99 & 0.07 & 0.86 & 2.24 & 55.93 & 718 & 88.0 \\
			IRIS (64) & 41.15 & 46.09 & 0.07 & 0.82 & 4.06 & 3.91 & 718& 88.0\\
			\hline
		\end{tabular}
	
	\caption{Reconstruction metrics for the radio-interferometry problem averaged over samples from the PROBES dataset which were not used to fine-tune our model, but which were used in pre-training the SBM in \cite{dia2025iris}. For both datasets, we compare PSNR for a single sample and for the estimated posterior mean (using the ergodic mean of $L-L_0=6$ samples for U-LATINO and 8 independent posterior samples for all other methods), LPIPS, SSIM and CFID (using a single posterior sample for each reconstruction). The average time per sample, GPU RAM and number of model parameter weights used to compute a single posterior sample are shown in the final column.} 
	\label{tab:RI_4h_results}
\end{table}

==> figures/kernels.tex <==

\begin{figure}
	\centering
	\begin{tikzpicture}
		% x
		\foreach \kcount in {0,...,6}
		{
			\node[inner sep = 0pt] (k\kcount) at (\kcount*\mywidth + 0.1*\kcount,0)
		 		{\includegraphics[width=\mywidthcm, height=\mywidthcm]{figures/MNIST_Deblurring/kernels/kernel_\kcount.png}};	
		 		
		 	\node[inner sep = 0pt] (kood\kcount) at (\kcount*\mywidth + 0.1*\kcount,-\mywidth - 1)
		 	{\includegraphics[width=\mywidthcm, height=\mywidthcm]{figures/MNIST_Deblurring/kernels/ood_/kernel_\kcount.png}};	
	 	}
 		\node[above=.1ex] (top) at (k3.north) {Training distribution};
 		
 		\node[above=.1ex] (top) at (kood3.north) {Out-of-distribution};
	\end{tikzpicture}
	\caption{Example motion blur kernels used for the MNIST experiment in \Cref{sec:numerics/mnist}. \textbf{Top}: in-distribution samples $\rvk\sim \mathcal{GP}(11, \lambda_\text{Matern} = 0.3, \sigma_\text{Matern}=0.25)$ used to train the models and for the evaluation in \Cref{sec:numerics/mnist}. \textbf{Bottom:} out-of-distribution kernels $\rvk\sim \mathcal{GP}(19, \lambda_\text{Matern} = 0.5, \sigma_\text{Matern}=0.4)$ covering a larger receptive field, with greater standard deviation and length-scale. For visual comparison, the in-distribution kernels are zero-padded to size $19\times19$.}
	\label{fig:kernels}
\end{figure}
